$U(1)$ local strings in generalized hybrid metric-Palatini gravity

In this work we will explore $U(1)$ local cosmic string solutions in the context of the generalized hybrid metric-Palatini theory of gravity in its scalar-tensor representation. Using a general static cylindrically symmetric metric to find the dynamical equations for this particular case, we will simplify the equations by imposing boost invariance along $t$ and $z$ directions. The strings properties are determined by both scalar fields and by the effective potential, function of the scalar fields. While for some forms of the potential, the dynamical equations can be solved exactly, for more general forms of the potential the solutions are found numerically. Several stable string configurations were found, whose basic parameters depend essentially on the effective field potential, and on the boundary conditions.

==> main-references.tex <==
%\cite{Zee:2003mt}
\bibitem{Zee:2003mt}
A.~Zee,
%``Quantum field theory in a nutshell,''
%180 citations counted in INSPIRE as of 11 Oct 2021

%\cite{Utiyama:1962sn}
\bibitem{Utiyama:1962sn}
R.~Utiyama and B.~S.~DeWitt,
%``Renormalization of a classical gravitational field interacting with quantized matter fields,''
J. Math. Phys. \textbf{3} (1962), 608-618
doi:10.1063/1.1724264
%414 citations counted in INSPIRE as of 28 Oct 2021

%\cite{Lovelock:1971yv}
\bibitem{Lovelock:1971yv}
D.~Lovelock,
%``The Einstein tensor and its generalizations,''
J. Math. Phys. \textbf{12} (1971), 498-501
doi:10.1063/1.1665613
%2000 citations counted in INSPIRE as of 28 Oct 2021

%\cite{Harko:2011nh}
\bibitem{Harko:2011nh}
T.~Harko, T.~S.~Koivisto, F.~S.~N.~Lobo and G.~J.~Olmo,
%``Metric-Palatini gravity unifying local constraints and late-time cosmic acceleration,''
Phys. Rev. D \textbf{85} (2012), 084016
doi:10.1103/PhysRevD.85.084016
[arXiv:1110.1049 [gr-qc]].
%138 citations counted in INSPIRE as of 18 Oct 2021

%\cite{Harko:2020ibn}
\bibitem{Harko:2020ibn}
T.~Harko and F.~S.~N.~Lobo,
%``Beyond Einstein\textquoteright{}s General Relativity: Hybrid metric-Palatini gravity and curvature-matter couplings,''
Int. J. Mod. Phys. D \textbf{29} (2020) no.13, 2030008
doi:10.1142/S0218271820300086
[arXiv:2007.15345 [gr-qc]].
%20 citations counted in INSPIRE as of 11 Oct 2021

%\cite{Vilenkin:2000jqa}
\bibitem{Vilenkin:2000jqa}
A.~Vilenkin and E.~P.~S.~Shellard,
%``Cosmic Strings and Other Topological Defects,''
%47 citations counted in INSPIRE as of 17 Oct 2021

%\cite{Olmo:2011uz}
\bibitem{Olmo:2011uz}
G.~J.~Olmo,
%``Palatini Approach to Modified Gravity: f(R) Theories and Beyond,''
Int. J. Mod. Phys. D \textbf{20} (2011), 413-462
doi:10.1142/S0218271811018925
[arXiv:1101.3864 [gr-qc]].
%462 citations counted in INSPIRE as of 29 Oct 2021

%\cite{Vilenkin:1981zs}
\bibitem{Vilenkin:1981zs}
A.~Vilenkin,
%``Gravitational Field of Vacuum Domain Walls and Strings,''
Phys. Rev. D \textbf{23} (1981), 852-857
doi:10.1103/PhysRevD.23.852
%997 citations counted in INSPIRE as of 25 Oct 2021

%\cite{ATLAS:2015yey}
\bibitem{ATLAS:2015yey}
G.~Aad \textit{et al.} [ATLAS and CMS],
%``Combined Measurement of the Higgs Boson Mass in $pp$ Collisions at $\sqrt{s}=7$ and 8 TeV with the ATLAS and CMS Experiments,''
Phys. Rev. Lett. \textbf{114} (2015), 191803
doi:10.1103/PhysRevLett.114.191803
[arXiv:1503.07589 [hep-ex]].
%1919 citations counted in INSPIRE as of 29 Oct 2021
